Conceiving Naturally After IVF: the effect of assisted reproduction on obstetric interventions and child health at birth

A growing share of the world's population is being born via assisted reproductive technology (ART), including in-vitro fertilisation (IVF). However, two concerns persist. First, ART pregnancies correlate with predictors of poor outcomes at birth--and it is unclear whether this relationship is causal. Second, the emotional and financial costs associated with ART-use might exacerbate defensive medical behaviour, where physicians intervene more than necessary to reduce the risk of adverse medical outcomes and litigation. We address the challenge of identifying the pure effect of ART-use on both maternal and infant outcomes at birth by leveraging exogenous variation in the success of ART cycles. We compare the obstetric outcomes for ART-conceived births with those of spontaneously-conceived births after a failed ART treatment. Moreover, we flexibly adjust for key confounders using double machine learning. We do this using clinical registry ART data and administrative maternal and infant data from New South Wales (NSW) between 2009-2017. We find that ART slightly decreases the risk of obstetric interventions, lowering the risk of a caesarean section and increasing the rate of spontaneous labour (+3.5 p.p.). Moreover, we find that ART has a statistically and clinically insignificant effect on infant health outcomes. Keywords: Fertility, Assisted reproduction, IVF, Caesarean Section, Obstetric, Infertility. JEL classification: I10, I12, I19.

==> Tables/anz_12_months_miss_table.tex <==
\begin{table}

\caption{\label{tab:tab:anz_12_month_miss_table}Test for observations missing at random.}
\centering
\begin{threeparttable}
\begin{tabular}[t]{lllll}
\toprule
 & No miss. & With miss. & Diff. & p-value\\
\midrule
Age & 34.9 & 35.09 & -0.19 & 0.0030\\
 & (4.56) & (4.51) & (0.065) & \\
No. of past unsuccessful cycles & 1.77 & 1.79 & -0.027 & 0.4092\\
 & (2.24) & (2.33) & (0.033) & \\
Maternal year of birth & 1977.82 & 1979.09 & -1.269 & 0.0000\\
 & (4.73) & (5.1) & (0.07) & \\
SEIFA & 3.49 & 3.46 & 0.026 & 0.1999\\
 & (1.41) & (1.39) & (0.02) & \\
Remoteness: major city & 0.89 & 0.9 & -0.003 & 0.5283\\
 & (0.31) & (0.31) & (0.004) & \\
Remoteness: inner regional & 0.09 & 0.09 & 0.001 & 0.7256\\
 & (0.28) & (0.28) & (0.004) & \\
Remoteness: outer regional & 0.02 & 0.02 & 0.001 & 0.6701\\
 & (0.13) & (0.13) & (0.002) & \\
Remoteness: remote and very remote & 0 & 0 & 0.001 & 0.3599\\
 & (0.05) & (0.04) & (0.001) & \\
Mother born in Australia & 0.66 & 0.65 & 0.012 & 0.0771\\
 & (0.47) & (0.48) & (0.007) & \\
No. of past pregnancies & 0.38 & 0.42 & -0.033 & 0.0006\\
 & (0.63) & (0.7) & (0.01) & \\
Diabetes mellitus & 0.01 & 0.01 & 0.006 & 0.0019\\
 & (0.11) & (0.08) & (0.002) & \\
Gestational diabetes & 0.09 & 0.08 & 0.013 & 0.0367\\
 & (0.29) & (0.27) & (0.006) & \\
Chronic hypertension & 0.01 & 0.01 & -0.001 & 0.5130\\
 & (0.1) & (0.1) & (0.001) & \\
Pre-eclampsia & 0.02 & 0.02 & -0.002 & 0.2391\\
 & (0.14) & (0.15) & (0.002) & \\
Gestational hypertension & 0.05 & 0.05 & 0.004 & 0.1804\\
 & (0.22) & (0.21) & (0.003) & \\
Smoked during pregnancy & 0.01 & 0.01 & 0.003 & 0.0696\\
 & (0.11) & (0.1) & (0.002) & \\
Endometriosis & 0.11 & 0.1 & 0.013 & 0.0032\\
 & (0.32) & (0.3) & (0.004) & \\
Other cause of infertility & 0.37 & 0.34 & 0.023 & 0.0006\\
 & (0.48) & (0.48) & (0.007) & \\
Male infertility & 0.42 & 0.31 & 0.114 & 0.0000\\
 & (0.49) & (0.46) & (0.007) & \\
Unexplained infertility & 0.29 & 0.29 & 0.004 & 0.5408\\
 & (0.46) & (0.45) & (0.006) & \\
\bottomrule
\end{tabular}
\begin{tablenotes}
\item \textit{Notes: } This table compares the mean values of each 
  variable in the population without missing observations and in that 
  with at least one missing observation.
\end{tablenotes}
\end{threeparttable}
\end{table}


==> Tables/anz_12_months_sample_balance_table.tex <==
\begin{table}

\caption{\label{tab:tab:cov_balance_anzard_12}Covariate balance table}
\centering
\begin{threeparttable}
\begin{tabular}[t]{lllllll}
\toprule
\multicolumn{1}{c}{ } & \multicolumn{2}{c}{Control} & \multicolumn{2}{c}{Treatment} & \multicolumn{2}{c}{Difference} \\
\cmidrule(l{3pt}r{3pt}){2-3} \cmidrule(l{3pt}r{3pt}){4-5} \cmidrule(l{3pt}r{3pt}){6-7}
Variable & Mean & Obs. & Mean & Obs. & Value & p-value\\
\midrule
Age & 36.78 & 935 & 34.75 & 12169 & 2.024 & 0.0000\\
 & (5.13) &  & (4.48) &  & (0.163) & \\
First cycle & 0.26 & 935 & 0.36 & 12169 & -0.099 & 0.0000\\
 & (0.44) &  & (0.48) &  & (0.015) & \\
No. of past unsuccessful cycles & 3.16 & 935 & 1.66 & 12169 & 1.501 & 0.0000\\
 & (2.53) &  & (2.18) &  & (0.073) & \\
Maternal year of birth & 1975.81 & 935 & 1977.98 & 12169 & -2.166 & 0.0000\\
 & (5.21) &  & (4.66) &  & (0.167) & \\
SEIFA & 3.49 & 935 & 3.49 & 12169 & 0.001 & 0.9776\\
 & (1.46) &  & (1.41) &  & (0.048) & \\
Remoteness: major city & 0.9 & 935 & 0.89 & 12169 & 0.011 & 0.2843\\
 & (0.3) &  & (0.31) &  & (0.011) & \\
Remoteness: inner regional & 0.07 & 935 & 0.09 & 12169 & -0.014 & 0.1058\\
 & (0.26) &  & (0.28) &  & (0.01) & \\
Remoteness: outer regional & 0.02 & 935 & 0.02 & 12169 & 0.005 & 0.3292\\
 & (0.15) &  & (0.13) &  & (0.005) & \\
Remoteness: remote and very remote & 0 & 935 & 0 & 12169 & -0.001 & 0.2863\\
 & (0.03) &  & (0.05) &  & (0.001) & \\
Mother born in Australia & 0.61 & 935 & 0.66 & 12169 & -0.053 & 0.0013\\
 & (0.49) &  & (0.47) &  & (0.016) & \\
Had past pregnancies & 0.4 & 935 & 0.32 & 12169 & 0.086 & 0.0000\\
 & (0.49) &  & (0.47) &  & (0.017) & \\
No. of past pregnancies & 0.53 & 935 & 0.37 & 12169 & 0.154 & 0.0000\\
 & (0.77) &  & (0.62) &  & (0.027) & \\
Diabetes mellitus & 0.01 & 935 & 0.01 & 12169 & 0.002 & 0.5584\\
 & (0.12) &  & (0.11) &  & (0.004) & \\
Gestational diabetes & 0.12 & 935 & 0.09 & 12169 & 0.033 & 0.0028\\
 & (0.33) &  & (0.29) &  & (0.011) & \\
Chronic hypertension & 0.01 & 935 & 0.01 & 12169 & 0.002 & 0.5394\\
 & (0.11) &  & (0.1) &  & (0.003) & \\
Pre-eclampsia & 0.02 & 935 & 0.02 & 12169 & -0.001 & 0.8918\\
 & (0.14) &  & (0.14) &  & (0.004) & \\
Gestational hypertension & 0.04 & 935 & 0.05 & 12169 & -0.008 & 0.2416\\
 & (0.2) &  & (0.22) &  & (0.007) & \\
Smoked during pregnancy & 0.02 & 935 & 0.01 & 12169 & 0.008 & 0.0996\\
 & (0.14) &  & (0.11) &  & (0.004) & \\
Endometriosis & 0.11 & 935 & 0.11 & 12169 & -0.008 & 0.4604\\
 & (0.31) &  & (0.32) &  & (0.011) & \\
Other cause of infertility & 0.38 & 935 & 0.37 & 12169 & 0.011 & 0.4964\\
 & (0.49) &  & (0.48) &  & (0.016) & \\
Male infertility & 0.35 & 935 & 0.43 & 12169 & -0.079 & 0.0000\\
 & (0.48) &  & (0.49) &  & (0.016) & \\
Unexplained infertility & 0.34 & 935 & 0.29 & 12169 & 0.055 & 0.0006\\
 & (0.48) &  & (0.45) &  & (0.016) & \\
\bottomrule
\end{tabular}
\begin{tablenotes}
\item \textit{Notes: } This table compares the covariate means of our treatment group\textemdash all ART births\textemdash and control group\textemdash spontaneous births conceived 3-to-12 months after a failed ART cycle. Each mean's standard errors is reported below it between parentheses. Taking the difference between the reported control and treated means typically returns a value inconsistent with the reported difference. This is due to rounding.
\end{tablenotes}
\end{threeparttable}
\end{table}


==> Tables/anz_12_months_sample_outcomes_table.tex <==
\begin{table}

\caption{\label{tab:tab:cov_balance_anzard_12}Outcome balance table for IVF sample (3-12 months)}
\centering
\begin{threeparttable}
\begin{tabular}[t]{lllllll}
\toprule
\multicolumn{1}{c}{ } & \multicolumn{2}{c}{Control} & \multicolumn{2}{c}{Treatment} & \multicolumn{2}{c}{Difference} \\
\cmidrule(l{3pt}r{3pt}){2-3} \cmidrule(l{3pt}r{3pt}){4-5} \cmidrule(l{3pt}r{3pt}){6-7}
Variable & Mean & Obs. & Mean & Obs. & Value & p-value\\
\midrule
Spontaneous labour & 0.3 & 1456 & 0.37 & 19636 & -0.067 & 0.0000\\
 & (0.46) &  & (0.48) &  & (0.013) & \\
Preterm spont. labour & 0.03 & 1456 & 0.04 & 19636 & -0.006 & 0.2331\\
 & (0.17) &  & (0.19) &  & (0.005) & \\
C-section & 0.55 & 1456 & 0.47 & 19646 & 0.083 & 0.0000\\
 & (0.5) &  & (0.5) &  & (0.014) & \\
Gestational age & 38.34 & 1456 & 38.45 & 19646 & -0.114 & 0.0848\\
 & (2.45) &  & (2.23) &  & (0.062) & \\
Pre-term birth & 0.09 & 1456 & 0.09 & 19646 & 0.006 & 0.4576\\
 & (0.29) &  & (0.28) &  & (0.008) & \\
APGAR1 & 8.36 & 1453 & 8.36 & 19607 & -0.005 & 0.9111\\
 & (1.57) &  & (1.52) &  & (0.041) & \\
APGAR5 & 8.86 & 1454 & 8.9 & 19608 & -0.04 & 0.1869\\
 & (1.1) &  & (1.05) &  & (0.03) & \\
Birth weight & 3260.16 & 1455 & 3303.95 & 19621 & -43.783 & 0.0081\\
 & (609.1) &  & (589.99) &  & (16.138) & \\
\bottomrule
\end{tabular}
\begin{tablenotes}
\item \textit{Notes: } Some notes la di da.
\end{tablenotes}
\end{threeparttable}
\end{table}


==> Tables/coef_table.tex <==
\begin{table}

  \caption{\label{tab:tab:ols}OLS: Effect of IVF conception on perinatal outcomes}
  \centering
  \begin{threeparttable}
    \begin{tabular}[t]{lllllll}
      \toprule
                                      & (1)       & (2)       & (3)       & (4)       & (5)       & (6)       \\
      \midrule
      \textit{Spontaneous labour}     & 0.042     & -0.017    & 0.028     & 0.008     & 0.028     & -0.017    \\
                                      & (0.016)   & (0.041)   & (0.02)    & (0.031)   & (0.025)   & (0.054)   \\
                                      & {}[0.006] & {}[0.668] & {}[0.157] & {}[0.786] & {}[0.263] & {}[0.756] \\
      \textit{Preterm spont. labour } & 0.009     & 0.01      & 0.014     & 0.006     & 0.014     & 0.006     \\
                                      & (0.006)   & (0.014)   & (0.008)   & (0.01)    & (0.01)    & (0.019)   \\
                                      & {}[0.156] & {}[0.481] & {}[0.075] & {}[0.587] & {}[0.157] & {}[0.751] \\
      \textit{C-section}              & -0.035    & 0.046     & -0.016    & 0.014     & 0.001     & -0.006    \\
                                      & (0.017)   & (0.04)    & (0.021)   & (0.031)   & (0.026)   & (0.053)   \\
                                      & {}[0.039] & {}[0.252] & {}[0.437] & {}[0.657] & {}[0.964] & {}[0.915] \\
      \textit{Gestational age}        & -0.077    & -0.154    & -0.145    & -0.07     & -0.222    & -0.086    \\
                                      & (0.086)   & (0.193)   & (0.12)    & (0.151)   & (0.14)    & (0.285)   \\
                                      & {}[0.375] & {}[0.423] & {}[0.225] & {}[0.642] & {}[0.113] & {}[0.764] \\
      \textit{Pre-term birth}         & 0.01      & 0.027     & 0.017     & 0.017     & 0.022     & 0.015     \\
                                      & (0.01)    & (0.02)    & (0.013)   & (0.016)   & (0.015)   & (0.027)   \\
                                      & {}[0.286] & {}[0.179] & {}[0.192] & {}[0.294] & {}[0.152] & {}[0.58]  \\
      \textit{APGAR1}                 & -0.001    & 0.202     & 0.02      & 0.134     & 0.002     & 0.364     \\
                                      & (0.057)   & (0.154)   & (0.078)   & (0.109)   & (0.091)   & (0.211)   \\
                                      & {}[0.983] & {}[0.192] & {}[0.795] & {}[0.218] & {}[0.981] & {}[0.085] \\
      \textit{APGAR5}                 & 0.012     & 0.149     & -0.017    & 0.126     & -0.031    & 0.306     \\
                                      & (0.041)   & (0.108)   & (0.055)   & (0.081)   & (0.065)   & (0.168)   \\
                                      & {}[0.764] & {}[0.169] & {}[0.756] & {}[0.117] & {}[0.634] & {}[0.068] \\
      \textit{Birth weight}           & 24.057    & -25.465   & 10.402    & 13.195    & -8.251    & 15.619    \\
                                      & (20.749)  & (47.036)  & (27.358)  & (36.889)  & (32.334)  & (67.219)  \\
                                      & {}[0.246] & {}[0.588] & {}[0.704] & {}[0.721] & {}[0.799] & {}[0.816] \\
                                      &           &           &           &           &           &           \\
      \textit{Obs. by treatment}      & 935/12169 & 153/3493  & 558/8311  & 268/4717  & 376/7199  & 91/2661   \\
      \bottomrule
    \end{tabular}
    \begin{tablenotes}
      \item Notes: This table reports average treatment effect
      estimates for the effect of an IVF conception on perinatal outcomes,
      estimated via OLS.
      Each column reports estimates for a different model specification.
      Each row reports effects for a different outcome.
      Column (1) reports the preferred estimates, which use all sample and
      confounders. Column (2): baseline if preterm equal 1.
      Column (3): first pregnancy and cycle. Column (4): first
      pregnancy. Column (5) first cycle.
      Column (6) restricts the sample to women at their first
      pregnancy and of less than 40 years of age. Column (7) further restricts to
      babies born at a gestational age less than 40 weeks.
      Column (8) shows the results for the full sample without using
      covariates. Standard errors are reported between parentheses, while p-values
      between square brackets.
    \end{tablenotes}
  \end{threeparttable}
\end{table}


==> Tables/dml_forest_ate_anzard_12.tex <==
\begin{table}

\caption{\label{tab:tab:dml_forest_ate_anzard_12}DML: ATE estimates of ART conception on obstetric outcomes}
\centering
\begin{threeparttable}
\begin{tabular}[t]{lrrrrrr}
\toprule
  & Coef. & s.e. & l-CI & r-CI & p-value & Obs.\\
\midrule
Spontaneous labour & 0.035 & 0.012 & 0.011 & 0.058 & 0.0034 & 13101\\
Preterm spont. labour & 0.005 & 0.005 & -0.004 & 0.014 & 0.2453 & 13101\\
C-section & -0.028 & 0.013 & -0.053 & -0.003 & 0.0258 & 13104\\
Gestational age & -0.038 & 0.062 & -0.160 & 0.084 & 0.5413 & 13104\\
Pre-term birth & 0.007 & 0.007 & -0.008 & 0.021 & 0.3608 & 13104\\
APGAR1 & 0.028 & 0.041 & -0.051 & 0.108 & 0.4865 & 13085\\
APGAR5 & 0.035 & 0.030 & -0.023 & 0.093 & 0.2404 & 13087\\
Birth weight & 18.953 & 15.248 & -10.932 & 48.838 & 0.2139 & 13089\\
\bottomrule
\end{tabular}
\begin{tablenotes}
\item \textit{Notes}: This tables reports our double machine learning estimates for the average 
treatment effect (ATE) of ART on obstetric outcomes. For each outcome (Column 1), we report the point estimate of the ATE (Column 2), its standard error (Column 3), its left and right 95\% confidence interval extrema (Columns 
4 and 5), its p-value (Column 6) and the number of observations (Column 7).
\end{tablenotes}
\end{threeparttable}
\end{table}


==> Tables/dml_forest_ate_anzard_12_trim_15.tex <==
\begin{table}

\caption{\label{tab:tab:dml_forest_ate_anzard_12_trim_15}DML: ATE estimates of ART conception on obstetric outcomes with trimming at 0.15}
\centering
\begin{threeparttable}
\begin{tabular}[t]{lrrrrrr}
\toprule
  & Coef. & s.e. & l-CI & r-CI & p-value & Obs.\\
\midrule
Spontaneous labour & 0.034 & 0.012 & 0.010 & 0.057 & 0.0050 & 13101\\
Preterm spont. labour & 0.005 & 0.005 & -0.004 & 0.014 & 0.2983 & 13101\\
C-section & -0.026 & 0.013 & -0.051 & -0.001 & 0.0418 & 13104\\
Gestational age & -0.030 & 0.063 & -0.153 & 0.093 & 0.6294 & 13104\\
Pre-term birth & 0.007 & 0.007 & -0.008 & 0.021 & 0.3622 & 13104\\
APGAR1 & 0.036 & 0.041 & -0.046 & 0.117 & 0.3899 & 13085\\
APGAR5 & 0.035 & 0.030 & -0.024 & 0.093 & 0.2488 & 13087\\
Birth weight & 18.621 & 15.402 & -11.567 & 48.809 & 0.2267 & 13089\\
\bottomrule
\end{tabular}
\begin{tablenotes}
\item \textit{Notes}: This tables reports our double machine learning estimates for the average 
treatment effect (ATE) of ART on obstetric outcomes, after trimming births with propensity scores 
under 0.15 and above 0.85. 
For each outcome (Column 1), we report the point estimate of the ATE (Column 2), its standard error (Column 3), its left and right 95\% confidence interval extrema (Columns 
4 and 5), its p-value (Column 6) and the number of observations (Column 7).
\end{tablenotes}
\end{threeparttable}
\end{table}


==> Tables/dml_forest_att_anzard_12.tex <==
\begin{table}

\caption{\label{tab:tab:dml_forest_att_anzard_12}DML: ATT estimates of IVF conception on perinatal outcomes}
\centering
\begin{threeparttable}
\begin{tabular}[t]{lrrrrrr}
\toprule
  & Coef. & s.e. & l-CI & r-CI & p-value & Obs.\\
\midrule
Spontaneous labour & 0.035 & 0.012 & 0.012 & 0.058 & 0.0027 & 13101\\
Preterm spont. labour & 0.006 & 0.004 & -0.003 & 0.014 & 0.1995 & 13101\\
C-section & -0.026 & 0.012 & -0.050 & -0.001 & 0.0392 & 13104\\
Gestational age & -0.028 & 0.061 & -0.148 & 0.092 & 0.6451 & 13104\\
Pre-term birth & 0.006 & 0.007 & -0.008 & 0.020 & 0.4011 & 13104\\
APGAR1 & 0.034 & 0.040 & -0.045 & 0.113 & 0.3960 & 13085\\
APGAR5 & 0.044 & 0.030 & -0.014 & 0.102 & 0.1377 & 13087\\
Birth weight & 20.188 & 15.082 & -9.373 & 49.748 & 0.1807 & 13089\\
\bottomrule
\end{tabular}
\begin{tablenotes}
\item \textit{Notes}: Some notes bidibibodibibù.
\end{tablenotes}
\end{threeparttable}
\end{table}

